Systematic Investigation of Sparse Perturbed Sharpness-Aware Minimization Optimizer

Deep neural networks often suffer from poor generalization due to complex and non-convex loss landscapes. Sharpness-Aware Minimization (SAM) is a popular solution that smooths the loss landscape by minimizing the maximized change of training loss when adding a perturbation to the weight. However, indiscriminate perturbation of SAM on all parameters is suboptimal and results in excessive computation, double the overhead of common optimizers like Stochastic Gradient Descent (SGD). In this paper, we propose Sparse SAM (SSAM), an efficient and effective training scheme that achieves sparse perturbation by a binary mask. To obtain the sparse mask, we provide two solutions based on Fisher information and dynamic sparse training, respectively. We investigate the impact of different masks, including unstructured, structured, and $N$:$M$ structured patterns, as well as explicit and implicit forms of implementing sparse perturbation. We theoretically prove that SSAM can converge at the same rate as SAM, i.e., $O(\log T/\sqrt{T})$. Sparse SAM has the potential to accelerate training and smooth the loss landscape effectively. Extensive experimental results on CIFAR and ImageNet-1K confirm that our method is superior to SAM in terms of efficiency, and the performance is preserved or even improved with a perturbation of merely 50\% sparsity. Code is available at https://github.com/Mi-Peng/Systematic-Investigation-of-Sparse-Perturbed-Sharpness-Aware-Minimization-Optimizer.

==> texfile/biography.tex <==

\begin{IEEEbiography}[{\includegraphics[width=1in,clip,keepaspectratio]{figs/biography/mipeng.jpg}}]{Peng Mi} received the B.Sc. degree in Electronic Information Engineering, from Xidian University, Xi'an, China in 2016. He is currently working toward the M.S. degree in artificial intelligence from the School of Informatics, Xiamen University, China. His research interests include computer vision and machine learning.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/biography/shenli.jpg}}]{Li Shen} 
received his Ph.D. in the School of Mathematics, at the South China University of Technology in 2017. He is currently a research scientist at JD Explore Academy, China. Previously, he was a research scientist at Tencent AI Lab in China. His research interests include theory and algorithms for large-scale convex/nonconvex/minimax optimization problems, and their applications in statistical machine learning, deep learning, reinforcement learning, and game theory.
\end{IEEEbiography}


\vspace{-1cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/biography/rentianhe.jpg}}]{Tianhe Ren} 
is an undergraduate student in the School of Information Science and Technology and is also a member of the Media Analytics and Computing Laboratory (MAC Lab) at Xiamen University, China.
\end{IEEEbiography}

\vspace{-1cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/biography/zhouyiyi.jpg}}]{Yiyi Zhou} 
(Member, IEEE) received the Ph.D. degree from Xiamen University, China, in 2019, under the supervision of Prof. Rongrong Ji. He was a Postdoctoral Research Search Fellow with Xiamen University from 2019 to 2022. He is currently an associate professor at School of Informatics and Institute of Artificial Intelligence of Xiamen University. His research interests include multimedia analysis and computer vision.
\end{IEEEbiography}

\vspace{-1cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,clip,keepaspectratio]{figs/biography/xutianshuo.jpg}}]{Tianshuo Xu} received the B.Sc. degree in intelligence science and technology from the School of Informatics, Xiamen University, Xiamen, China, in 2016. He is currently working toward the M.S. degree in artificial intelligence from the School of Informatics, Xiamen University, China. His research interests include computer vision and machine learning.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/biography/sunxiaoshuai.jpg}}]{Xiaoshuai Sun} 
(Senior Member, IEEE) received the B.S. degree in Computer Science from Harbin Engineering University in 2007, and the M.S. \& Ph.D. degree in Computer Science and Technology at Harbin Institute of Technology in 2009 and 2015 respectively. He is currently an associate professor at the School of Informatics, Xiamen University, China. His research interests include computer vision, pattern recognition, and multimedia analysis. He was a recipient of the best Ph.D thesis award in Harbin Institute of Technology (2015) and also a winner of Microsoft Research Fellowship (2011). He owns 4 authorized patents and has authored over 100 papers in referred journals and conferences, including TPAMI, TIP, CVPR, ICCV, NeurIPS, IJCAI, AAAI and ACM MM. 
\end{IEEEbiography}

\vspace{-1cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,clip,keepaspectratio]{figs/biography/tongliangliu.png}}]{Tongliang Liu} is the Director of Sydney AI Centre at the University of Sydney. He is also heading the Trustworthy Machine Learning Laboratory. He is broadly interested in the fields of trustworthy machine learning and its interdisciplinary applications, with a particular emphasis on learning with noisy labels, adversarial learning, transfer learning, unsupervised learning, and statistical deep learning theory. He has authored and co-authored more than 100 research articles including ICML, NeurIPS, ICLR, CVPR, ICCV, ECCV, AAAI, IJCAI, KDD, IEEE T-PAMI, T-NNLS, and T-IP. He is/was a (senior-) meta reviewer for many conferences, such as ICML, NeurIPS, ICLR, UAI, AAAI, IJCAI, and KDD. He is a recipient of Discovery Early Career Researcher Award (DECRA) from Australian Research Council (ARC); the Cardiovascular Initiative Catalyst Award by the Cardiovascular Initiative; and was named in the Early Achievers Leaderboard of Engineering and Computer Science by The Australian in 2020.
\end{IEEEbiography}

\vspace{-1cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,clip,keepaspectratio]{figs/biography/jirongrong.jpeg}}]{Rongrong Ji} (Senior Member, IEEE)
is currently a Nanqiang distinguished professor at Xiamen University, China, the deputy director of the Office of Science and Technology at Xiamen University, China, and the director of Media Analytics and Computing Lab. He was awarded as the National Science Foundation for Excellent Young Scholars (2014), the National Ten Thousand Plan for Young Top Talents (2017), and the National Science Foundation for Distinguished Young Scholars (2020). His research interests include computer vision, multimedia analysis, and machine learning. He has published more than 50 papers in ACM/IEEE Transactions, including the IEEE Transactions on Pattern Analysis and Machine Intelligence and the International Journal of Computer Vision, and more than 100 full papers on top-tier conferences, such as CVPR and NeurIPS. His publications have got more than 10K citations in Google Scholar. He was the recipient of the Best Paper Award of ACM Multimedia 2011. He has served as area chair in top-tier conferences such as CVPR and ACM Multimedia. He is also an advisory member for Artificial Intelligence Construction in the Electronic Information Education Committee of the National Ministry of Education.
\end{IEEEbiography}


\vspace{-1cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/biography/DachengTao.png}}]{Dacheng Tao}
% or if you just want to reserve a space for a photo:
% \begin{IEEEbiography}{Michael Shell}
(Fellow, IEEE) received a BEng degree from the University of Science and Technology of China (USTC), the MPhil degree from the Chinese University of Hong Kong (CUHK), and a Ph.D. from the University of London (UoL). Currently, of Computer Science and ARC Laureate Fellow in the School of Computer Science and the Faculty of Engineering, and the Inaugural Director of the UBTECH Sydney Artificial Intelligence Centre, at The University of Sydney. His research results in artificial intelligence have been expounded in one monograph and 200+ publications at prestigious journals and prominent conferences, such as IEEE TPAMI, IJCV, AIJ, AAAI, IJCAI, NeurIPS, ICML, CVPR, ICCV, ECCV, ICDM, and KDD, with several best paper awards. He received the 2018 IEEE ICDM Research Contributions Award and the 2015 Australian Museum Scopus-Eureka Prize. He is a Fellow of the IEEE, ACM, AAAS, and the Australian Academy of Science.
\end{IEEEbiography}
